The James construction and $\pi_4(\mathbb{S}^3)$ in homotopy type theory

In the first part of this paper we present a formalization in Agda of the James construction in homotopy type theory. We include several fragments of code to show what the Agda code looks like, and we explain several techniques that we used in the formalization. In the second part, we use the James construction to give a constructive proof that $\pi_4(\mathbb{S}^3)$ is of the form $\mathbb{Z}/n\mathbb{Z}$ (but we do not compute the $n$ here).

==> code/JSSRec.tex <==
\begin{code}
\\[-\baselineskip]
\>\AgdaKeyword{module} \AgdaModule{\_} \AgdaSymbol{\{}\AgdaBound{l}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{)} \AgdaSymbol{\{}\AgdaBound{X} \AgdaSymbol{:} \AgdaFunction{Type} \AgdaBound{l}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{(}\AgdaBound{ι*} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaBound{n} \AgdaSymbol{→} \AgdaBound{X}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{(}\AgdaBound{α*} \AgdaSymbol{:} \AgdaBound{A} \AgdaSymbol{→} \AgdaFunction{JS} \AgdaBound{n} \AgdaSymbol{→} \AgdaBound{X}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{(}\AgdaBound{β*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{α*} \AgdaBound{⋆A} \AgdaBound{x} \AgdaDatatype{==} \AgdaBound{ι*} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{(}\AgdaBound{γ*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{a} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{α*} \AgdaBound{a} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{α} \AgdaBound{n} \AgdaBound{a} \AgdaBound{x}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{(}\AgdaBound{η*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{Square} \AgdaSymbol{(}\AgdaBound{γ*} \AgdaBound{⋆A} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{β*} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{JSS-rec} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{X}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{JSS-rec} \AgdaSymbol{=} \AgdaFunction{Pushout-rec} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaBound{α*}\AgdaSymbol{)} \AgdaBound{ι*} \AgdaFunction{JSS-rec-push} \<[54]%
\>[54]\AgdaKeyword{module} \AgdaModule{\_} \AgdaKeyword{where}\<%
\\[-0.1cm]
%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{JSS-rec-push} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{c} \AgdaSymbol{:} \AgdaFunction{JS.X} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{uncurry} \AgdaBound{α*} \AgdaSymbol{(}\AgdaFunction{JS.f} \AgdaBound{n} \AgdaBound{c}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{JS.g} \AgdaBound{n} \AgdaBound{c}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{JSS-rec-push} \AgdaSymbol{=} \AgdaPostulate{Pushout-elim} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaBound{γ*}\AgdaSymbol{)} \AgdaBound{β*} \AgdaSymbol{(λ} \AgdaBound{x} \AgdaSymbol{→} \AgdaFunction{↓-='-from-square} \AgdaSymbol{(}\AgdaFunction{α-f-push} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{ι-g-push} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{η*} \AgdaBound{x}\AgdaSymbol{))} \<[107]%
\>[107]\AgdaKeyword{where}\<%
\\[-0.1cm]
%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{α-f-push} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{ap} \AgdaSymbol{((}\AgdaFunction{uncurry} \AgdaBound{α*}\AgdaSymbol{)} \AgdaFunction{∘} \AgdaSymbol{(}\AgdaFunction{JS.f} \AgdaBound{n}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaInductiveConstructor{idp}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{α-f-push} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{ap-∘} \AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaFunction{∙} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaBound{α*}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{push-β} \AgdaBound{x}\AgdaSymbol{)}\<%
\\[-0.1cm]
%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{ι-g-push} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaBound{ι*} \AgdaFunction{∘} \AgdaSymbol{(}\AgdaFunction{JS.g} \AgdaBound{n}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaFunction{ap} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{ι-g-push} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{ap-∘} \AgdaBound{ι*} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaFunction{∙} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaBound{ι*}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{push-β} \AgdaBound{x}\AgdaSymbol{)}\<%
\\[-0.1cm]
%
\\
\>\AgdaKeyword{module} \AgdaModule{\_} \AgdaSymbol{\{}\AgdaBound{l}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{)} \AgdaSymbol{\{}\AgdaBound{X} \AgdaSymbol{:} \AgdaFunction{Type} \AgdaBound{l}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{ι*} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaBound{n} \AgdaSymbol{→} \AgdaBound{X}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{α*} \AgdaSymbol{:} \AgdaBound{A} \AgdaSymbol{→} \AgdaFunction{JS} \AgdaBound{n} \AgdaSymbol{→} \AgdaBound{X}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{β*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{α*} \AgdaBound{⋆A} \AgdaBound{x} \AgdaDatatype{==} \AgdaBound{ι*} \AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{γ*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{a} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{α*} \AgdaBound{a} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{α} \AgdaBound{n} \AgdaBound{a} \AgdaBound{x}\AgdaSymbol{)\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{η*} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{Square} \AgdaSymbol{(}\AgdaBound{γ*} \AgdaBound{⋆A} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaBound{ι*} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{β*} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{private} \AgdaFunction{JSS-rec'} \AgdaSymbol{=} \AgdaFunction{JSS-rec} \AgdaBound{n} \AgdaBound{ι*} \AgdaBound{α*} \AgdaBound{β*} \AgdaBound{γ*} \AgdaBound{η*}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{private} \AgdaFunction{JSS-rec-push'} \AgdaSymbol{=} \AgdaFunction{JSS-rec-push} \AgdaBound{n} \AgdaBound{ι*} \AgdaBound{α*} \AgdaBound{β*} \AgdaBound{γ*} \AgdaBound{η*}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{β-β} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{JS} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{ap} \AgdaFunction{JSS-rec'} \AgdaSymbol{(}\AgdaFunction{β} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaBound{β*} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{β-β} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{push-β} \AgdaSymbol{(}\AgdaPostulate{inr} \AgdaBound{x}\AgdaSymbol{)}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{γ-β} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{a} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{ap} \AgdaFunction{JSS-rec'} \AgdaSymbol{(}\AgdaFunction{γ} \AgdaBound{n} \AgdaBound{a} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaBound{γ*} \AgdaBound{a} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{γ-β} \AgdaBound{a} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{push-β} \AgdaSymbol{(}\AgdaPostulate{inl} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{x}\AgdaSymbol{))}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{η-β} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{FlatCube} \AgdaSymbol{(}\AgdaFunction{ap-square} \AgdaFunction{JSS-rec'} \AgdaSymbol{(}\AgdaFunction{η} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaSymbol{(}\AgdaBound{η*} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaSymbol{(}\AgdaFunction{γ-β} \AgdaBound{⋆A} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaInductiveConstructor{idp}\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaSymbol{(}\AgdaFunction{∘-ap} \AgdaFunction{JSS-rec'} \AgdaPostulate{inr} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaSymbol{(}\AgdaFunction{β-β} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{η-β} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{adapt-flatcube} \AgdaFunction{∙idp}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{(}\AgdaField{\&} \AgdaFunction{coh} \AgdaSymbol{(}\AgdaFunction{ap-∘3} \AgdaFunction{JSS-rec'} \AgdaPostulate{inl} \<[53]%
\>[53]\AgdaSymbol{\_} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{natural-square} \AgdaSymbol{(}\AgdaFunction{ap-∘} \AgdaFunction{JSS-rec'} \AgdaPostulate{inl}\AgdaSymbol{)} \<[102]%
\>[102]\AgdaSymbol{(}\AgdaFunction{push-β} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaSymbol{(}\AgdaFunction{ap-∘} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaFunction{JSS-rec'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaPostulate{inl}\AgdaSymbol{)} \<[147]%
\>[147]\AgdaSymbol{\_))} \AgdaSymbol{(}\AgdaFunction{ap-∙} \AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{\_))}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{(}\AgdaField{\&} \AgdaFunction{coh} \AgdaSymbol{(}\AgdaFunction{ap-∘3} \AgdaFunction{JSS-rec'} \AgdaPostulate{inr} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{natural-square} \AgdaSymbol{(}\AgdaFunction{ap-∘} \AgdaFunction{JSS-rec'} \AgdaPostulate{inr}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{push-β} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaSymbol{(}\AgdaFunction{ap-∘} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaFunction{JSS-rec'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaPostulate{inr}\AgdaSymbol{)} \AgdaSymbol{\_))} \AgdaSymbol{(}\AgdaFunction{ap-∙} \AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{\_))}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaFunction{∙idp}\<%
\\
\>[0]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{((}\AgdaField{\&} \AgdaSymbol{(}\AgdaFunction{ap-square-natural-square} \AgdaFunction{JSS-rec'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaPostulate{push} \AgdaInductiveConstructor{idp} \AgdaInductiveConstructor{idp}\<%
\\
\>[0]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{/∙³} \AgdaField{\&} \AgdaFunction{natural-square-homotopy} \AgdaFunction{push-β} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{∙fc} \AgdaField{\&} \AgdaFunction{natural-square==} \AgdaFunction{JSS-rec-push'} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaInductiveConstructor{idp}\<%
\\
\>[0]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{∙³/} \AgdaFunction{natural-square-β} \AgdaFunction{JSS-rec-push'} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{push-βd} \AgdaBound{x}\AgdaSymbol{)))} \<[71]%
\>[71]\AgdaKeyword{where}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{coh} \AgdaSymbol{:} \AgdaRecord{Coh} \AgdaSymbol{(\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaFunction{Type} \AgdaBound{l}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaBound{d} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{p} \AgdaSymbol{:} \AgdaBound{a} \AgdaDatatype{==} \AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{q} \AgdaSymbol{:} \AgdaBound{a} \AgdaDatatype{==} \AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{r} \AgdaSymbol{:} \AgdaBound{b} \AgdaDatatype{==} \AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{s} \AgdaSymbol{:} \AgdaBound{c} \AgdaDatatype{==} \AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{sq1} \AgdaSymbol{:} \AgdaDatatype{Square} \AgdaBound{p} \AgdaBound{q} \AgdaBound{r} \AgdaBound{s}\AgdaSymbol{)}\<%
\\
\>[4]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{t} \AgdaSymbol{:} \AgdaBound{c} \AgdaDatatype{==} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{u} \AgdaSymbol{:} \AgdaBound{d} \AgdaDatatype{==} \AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{v} \AgdaSymbol{:} \AgdaBound{e} \AgdaDatatype{==} \AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{sq2} \AgdaSymbol{:} \AgdaDatatype{Square} \AgdaBound{s} \AgdaBound{t} \AgdaBound{u} \AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[4]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{\{}\AgdaBound{ru} \AgdaSymbol{:} \AgdaBound{b} \AgdaDatatype{==} \AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{ru=} \AgdaSymbol{:} \AgdaBound{ru} \AgdaDatatype{==} \AgdaBound{r} \AgdaFunction{∙} \AgdaBound{u}\AgdaSymbol{)}\<%
\\
\>[4]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaInductiveConstructor{idp} \AgdaFunction{∙} \AgdaFunction{!} \AgdaSymbol{(}\AgdaBound{p} \AgdaFunction{∙} \AgdaBound{ru}\AgdaSymbol{)} \AgdaFunction{∙} \AgdaBound{q} \AgdaFunction{∙} \AgdaBound{t} \AgdaDatatype{==} \AgdaFunction{!} \AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{coh} \AgdaSymbol{=} \AgdaFunction{path-induction}\<%
\end{code}


==> code/defge.tex <==
\begin{code}
\\[-\baselineskip]
\>\AgdaFunction{γ} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{a} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{α} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaBound{a} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{α} \AgdaBound{n} \AgdaBound{a} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{γ} \AgdaBound{n} \AgdaBound{a} \AgdaBound{x} \AgdaSymbol{=} \AgdaPostulate{push} \AgdaSymbol{(}\AgdaPostulate{inl} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{x}\AgdaSymbol{))}\<%
\\[-0.1cm]
%
\\
\>\AgdaFunction{η} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{J} \AgdaBound{n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaDatatype{Square} \AgdaSymbol{(}\AgdaFunction{γ} \AgdaBound{n} \AgdaBound{⋆A} \AgdaBound{x}\AgdaSymbol{)} \AgdaInductiveConstructor{idp} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{β} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{η} \AgdaBound{n} \AgdaBound{x} \AgdaSymbol{=} \AgdaFunction{natural-square} \AgdaPostulate{push} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaFunction{α-f-push} \AgdaFunction{ι-g-push} \<[56]%
\>[56]\AgdaKeyword{where}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{α-f-push} \AgdaSymbol{:} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaSymbol{(}\AgdaFunction{α} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{))} \AgdaFunction{∘} \AgdaFunction{JS.f} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaInductiveConstructor{idp}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{α-f-push} \AgdaSymbol{=} \<[14]%
\>[14]\AgdaFunction{ap-∘} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaSymbol{(}\AgdaFunction{α} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{JS.f} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaFunction{∙} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{uncurry} \AgdaSymbol{(}\AgdaFunction{α} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{))))} \AgdaSymbol{(}\AgdaFunction{push-β} \AgdaSymbol{\_)}\<%
\\[-0.1cm]
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{ι-g-push} \AgdaSymbol{:} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)} \AgdaFunction{∘} \AgdaFunction{JS.g} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)} \AgdaDatatype{==} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{β} \AgdaBound{n} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{ι-g-push} \AgdaSymbol{=} \<[14]%
\>[14]\AgdaFunction{ap-∘} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{JS.g} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaPostulate{push} \AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaFunction{∙} \AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ap} \AgdaSymbol{(}\AgdaFunction{ι} \AgdaSymbol{(}\AgdaInductiveConstructor{S} \AgdaBound{n}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{push-β} \AgdaSymbol{\_)}\<%
\end{code}

